On the Robustness of Temporal Vision-Language Models for Surgical Endoscopy Videos

Temporal vision-language models (TVLMs) offer a reusable, prompt-based interface for surgical video understanding, yet, their robustness under clinically realistic acquisition artifacts in endoscopy remains insufficiently characterized. In practice, degradations such as defocus, haze, motion blur, noise, cautery smoke, and packet loss introduce structured distribution shifts which may compromise video-text alignment. We study the robustness of temporal VLMs under such shifts caused by corruptions in clip frames. We introduce Endo-C6, a compact corruption benchmark of six endoscopy-realistic perturbations evaluated at a fixed high severity, and apply it to public Gastrointestinal (GI) endoscopy and laparoscopic cholecystectomy videos. Under a standardized prompt protocol, we benchmark 3 recent surgical TVLM baselines and analyze robustness in both mean and worst-case settings, spanning 294 dataset-level evaluations. Finally, we present RobustEndoCLIP, obtained by few-shot parameter-efficient tuning with VeRA, outperforming existing TVLM baselines. Our findings show that off-the-shelf TVLMs can exhibit severe worst-case collapse under endoscopy-specific corruptions, whereas lightweight few-shot adaptation can substantially improve corrupted performance and robustness without changing the prompt-based interface. We expect Endo-C6 to support standardized robustness reporting and promote more reliable clinical vision-language systems.

==> Tables/number_of_shots.tex <==
\begin{table}[t]
\centering
\caption{{Label budget scaling.} RobustEndoCLIP (VeRA) robustness vs.\ labeled fraction of the \emph{clean} training set, reported across datasets under Endo-C6. We report Clean, Mean-C, Worst-C, and robustness gap $\Delta=\text{Clean}-\text{Mean-C}$.}
\label{tab:shot_scaling}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc|cccc|cccc}
\toprule
& \multicolumn{4}{c}{{CholecT50}} & \multicolumn{4}{c}{{Kvasir}} & \multicolumn{4}{c}{{TEMSET-24K}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
{Label budget} &
{Clean} & {Mean} & {Worst} & $\boldsymbol{\Delta}$ &
{Clean} & {Mean} & {Worst} & $\boldsymbol{\Delta}$ &
{Clean} & {Mean} & {Worst} & $\boldsymbol{\Delta}$ \\
\midrule
0\% & 40.21 & 12.57 & 7.08 & 27.64 & 13.75 & 12.38 & 9.50 & 1.37 & 2.82 & 3.86 & 2.07 & -1.04 \\
4\%            & 48.36 & 33.82 & 13.29 & 14.54 & 22.75 & 18.20 & 10.92 & 4.55 & 27.00 & 25.72 & 19.02 & 1.28 \\
8\%            & 47.83 & 35.54 & 14.85 & 12.29 & 34.00 & 23.70 & 11.75 & 10.30 & 26.90 & 26.64 & 17.59 & 0.26 \\
\rowcolor{myblue!40}
16\%           & 47.06 & 38.29 & 16.83 & 8.77 & 36.50 & 22.20 & 11.42 & 14.30 & 26.67 & 26.89 & 19.98 & -0.22 \\
\bottomrule
\end{tabular}}
\end{table}


==> Tables/stride_percentage.tex <==
% \begin{table*}[t]
% \centering
% \caption{\textbf{Corruption stride ablation on CholecT50.} Robustness under different corruption injection strides (example: apply burst corruption on 50\% of the frames vs on all frames) under Endo-C6\vspace{0.1cm}.}
% \label{tab:corruption_stride}
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.08}
% \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{lc|cccccc|cc|c}
% \toprule
% {Stride setting} &
% {Clean} &
% {Defocus} &
% {Fog} &
% {Shot} &
% {Motion} &
% {Packet} &
% {Smoke} &
% {Mean-C\vspace{0.1cm}} &
% {Worst-C\vspace{0.1cm}} &
% $\boldsymbol{\Delta}$ \\
% \midrule
% 50\% Frames  & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD \\
% 100\% Frames & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD & \TBD \\
% \bottomrule
% \end{tabular}}
% \end{table*}
